Probing the haze in the atmosphere of HD 189733b with HST/WFC3 transmission spectroscopy

We present Hubble Space Telescope near-infrared transmission spectroscopy of the transiting exoplanet HD 189733b, using Wide Field Camera 3. This consists of time-series spectra of two transits, used to measure the wavelength dependence of the planetary radius. These observations aim to test whether the Rayleigh scattering haze detected at optical wavelengths extends into the near-infrared, or if it becomes transparent leaving molecular features to dominate the transmission spectrum. Due to saturation and non-linearity affecting the brightest (central) pixels of the spectrum, light curves were extracted from the blue and red ends of the spectra only, corresponding to wavelength ranges of 1.099-1.168 um and 1.521-1.693 um, respectively, for the first visit, and 1.082-1.128 um and 1.514-1.671 um for the second. The light curves were fitted using a Gaussian process model to account for instrumental systematics whilst simultaneously fitting for the transit parameters. This gives values of the planet-to-star radius ratio for the blue and red light curves of 0.15650\pm0.00048 and 0.15634\pm0.00032, respectively, for visit one and 0.15716\pm0.00078 and 0.15630\pm0.00037 for visit 2 (using a quadratic limb darkening law). The planet-to-star radius ratios measured in both visits are consistent, and we see no evidence for the drop in absorption expected if the haze that is observed in the optical becomes transparent in the infrared. This tentatively suggests that the haze dominates the transmission spectrum of HD 189733b into near-infrared wavelengths, although more robust observations are required to provide conclusive evidence.

==> PaxHeader/Gibson_WFC_HD189733.tex <==
17 gid=784332012
16 uid=11790662
20 ctime=1328021070
20 atime=1328021070
38 LIBARCHIVE.creationtime=1327691657
24 SCHILY.dev=754974724
24 SCHILY.ino=228314447
18 SCHILY.nlink=1

